How Much Demand Flexibility Could Have Spared Texas from the 2021 Outage?

The February 2021 Texas winter power outage has led to hundreds of deaths and billions of dollars in economic losses, largely due to the generation failure and record-breaking electric demand. In this paper, we study the scaling-up of demand flexibility as a means to avoid load shedding during such an extreme weather event. The three mechanisms considered are interruptible load, residential load rationing, and incentive-based demand response. By simulating on a synthetic but realistic large-scale Texas grid model along with demand flexibility modeling and electricity outage data, we identify portfolios of mixing mechanisms that exactly avoid outages, which a single mechanism may fail due to decaying marginal effects. We also reveal a complementary relationship between interruptible load and residential load rationing and find nonlinear impacts of incentive-based demand response on the efficacy of other mechanisms.

==> sec/2_Flexibility.tex <==
\section{Demand Flexibility in Energy Portfolio Transition}
\subsection*{Formulation of Demand Flexibility}
% \paragraph{Literature review of demand flexibility} \textcolor{blue}{This paragraph should format and explain the potential benefit of enhanced demand flexibility.}
In the tide of energy portfolio transition towards decarbonization, electricity grids face challenges of insufficient security and adequacy due to factors such as deepening penetration of intermittent renewables, rapid proliferation of electric vehicles, frequent occurrence of extreme weather, and so on.
% Note that demand flexibility in this paper refers to the overall capability in electricity demand sectors of altering end-use consumption by either contractual or voluntary mechanisms to maintain system's reliability and efficiency~\cite{zhou2021electrification}.

In this paper, demand flexibility is described from three technical aspects that depend on control functions, including \textit{response time}, \textit{duration}, and \textit{uncertainty}~\cite{akrami2019power}. Accordingly we propose a general formulation of demand flexibility sources as follows,
\begin{subequations}\label{eq:DR_def}
\begin{align}
    &R_{\text{min}}\leq R_t \leq R_{\text{max}},\\
    &\frac{dP_t}{dt}=R_t,\\
    &0\leq P_t \leq P_{\text{max}},\\
    &T_{\text{min}}\leq T \leq T_{\text{max}},
\end{align}
\end{subequations}
where $R_t$ represents the ramping rate at time $t$, $R_{\text{max}}$ means the maximal response rate, the absolute value of $R_{\text{min}}$ means the maximal restoration rate, $P_t$ means the reduced load power, $P_{\text{max}}$ means the maximum capacity provided by the demand flexibility source, and $T$, $T_{\text{min}}$, and $T_{\text{max}}$ represent actual, minimal and maximal activating duration, respectively. Specifically,  $P_{\text{max}}$ is constant for deterministic demand response sources, while it can be a random variable following some distribution $\mathop{\mathbb{P}}$ in stochastic cases.

% In the remaining part of the paper, we will present several featured types of demand response schemes represented by such formulation regardless of their distinct formats and implementation. Particularly, we will elaborate the definition in Section~\ref{subsec:DR_schemes} and present detailed modelling in Section~\ref{sec:quantification}.


\subsection*{Introduction of Demand Response Programs}\label{subsec:DR_schemes}
Demand flexibility is concretized by demand response programs of various forms that can change the energy consumption of end-use customers from normal patterns in response to certain commands or signals~\cite{balijepalli2011review}. 
In most electricity markets across the U.S., demand response providers (DRPs) are allowed to collect demand response commitments from customers and are treated as “virtual generators” that can participate in real-time markets and/or provide operating reserves in the ancillary services markets~\cite{Loadresource, Nyiso, Caiso}.
Specifically, load resources in ERCOT can participate in the ancillary service market, which includes regulation up/down, non-spinning reserve service, and responsive reserve service (RRS). The bulk part of these services is attributed to the RRS, which can be automatically interrupted by under-frequency relays (UFRs) or manually cut-off within a ten-minute notice~\cite{habib2021improving}. During the most difficult hours of the Texas power outage, the maximum load reduction from load resources providing reserve was over 1,400 MW throughout the blackout event~\cite{king2021timeline}.

% \begin{itemize}
% \item Contractual Load Management

% \textbf{Load Resources (Ancillary Services Market):}
% Besides participating in ERCOT's day-ahead and real-time markets, load resources can also provide ancillary services  if they are willing to curtail or shift load upon ERCOT's request. This includes Regulation Up/Down, Non-Spinning Reserve Service, and Responsive Reserve Service (RRS). The bulk part of these services is coming from the RRS, which requires installing Under Frequency Relay (UFR)
% that opens the load feeder breaker on automatic detection of an under frequency condition. These loads are also required to be
% manually interrupted within a 10-minute notice \cite{habib2021improving}

% 
% February 19 \cite{king2021timeline}. Despite the extreme need for more reserve, this is below the average of 1,548 MW resource provided in January 2021 \cite{king2021timeline}, and the majority of this amount comes from the resources providing RRS.

% \textbf{Emergency Response Service (ERS):}
% ERCOT procures ERS four times during the ERS calendar year, and according to two different response times—thirty minutes (ERS-30) and ten minutes (ERS-10). 

% \item Incentive-based Demand Response :
% (Transmission/Distribution Service Provider (TDSP) Load Management Programs) 
% \item Load Rationing :
% \end{itemize}


% In another attempt to reduce the system load, the Emergency Response Service (ERS) program was also activated by ERCOT during the winter storm. While the participating loads in the ERS program provided demand reduction well above their obligations, the generation units met less than half of their obligation of around 300 MW in the early hours of February 15. Still, the ERS program achieved its targeted level of demand reduction of roughly 1,100 MW during the morning of February 15 \cite{FERC2021}.

To assess the effects of demand flexibility against extreme weather conditions in future, we focus on three featured types of demand response programs, including \textit{interruptible load}, \textit{residential load rationing}, and \textit{incentive-based demand response}, of which the definitions are elaborated as follows.


\paragraph{\textbf{Interruptible load}} We refer interruptible load to a type of contractual demand response programs that can interrupt large-size commercial and industry loads to arbitrary extent within a short period upon requests, such as existing demand-side reserves in ERCOT.


\paragraph{\textbf{Residential load rationing}} We refer residential load rationing to a type of contractual demand response programs that can restrict residential electricity consumption during energy scarcity, which is potentially implemented by smart meters that have access to appliance control. Note that although both interruptible load and residential load rationing are firm demand response programs with no uncertainty, being fulfilled on different load sectors may cause distinct impacts.


\paragraph{\textbf{Incentive-based demand response}} We refer incentive-based demand response to a type of voluntary demand response programs that can exploit the elasticity of residential loads by impelling voluntary and stochastic load shifting in response to \textit{Energy Coupon}-like bonus incentive~\cite{zhong2012coupon,xia2017energycoupon,ming2020prediction} rather than price-based incentive\footnote{Price-based incentive aiming at load reduction or shifting is not effective during this blackout event, as wholesale market nodal prices attained the maximum.}.

Despite the heterogeneous forms, these demand response programs can be represented in the proposed general formulation (Eq.~\eqref{eq:DR_def}) (see more details in Methods). 
% of which the parameters are presented in Table~\ref{tab:DR_parameters}, and we set $T_\text{min}$ as $0$ consistently\footnote{We assume no limitation on minimal activating time, which notwithstanding can be adjusted in future work such as electricity storage-related study.}. (XXXXXXXXXXXXXXX)
% Based on the proposed modelling formulation and parameters, the effects of demand response portfolios aiding in electricity scarcity will be quantified in Section~\ref{sec:quantification}.
 
 

==> sec/3_Model_and_Data.tex <==
\begin{figure*}[thpb!]
	\centering
	\includegraphics[width=1\textwidth]{fig/data_and_model.pdf}
	\caption{Visualization of load profiling and synthetic simulation models over weather zones. (a) The stacked plot presents the estimated load percentages of three load sectors in weather zones, which shows the significant rising proportion of residential load sectors with the winter storm incoming (starting from February 11). The dashed red vertical lines indicate the beginning and end of the blackout event. (b) It shows the topology of the synthetic Texas grid adapted from~\cite{wu2021open}, where the width is proportional to the transmission line capacity.}
	\label{fig:data_and_model}
\end{figure*}


\section*{Open-source Simulation Model and Data}
\subsection*{Load Profile Estimation}
To improve the fidelity of our simulation and model different demand response proposals in richer detail, we further decompose the ERCOT weather-zone level total load data into 3 sectors: residential, commercial/industrial and municipal. We estimate a percentage share of the sectors in the total load of each weather zone (see Methods), at each hour in February 2021 using the ERCOT backcasted actual load profile~\cite{ERCOT_load_profiling}, which contains normalized daily load profiles from each of the 8 weather zones in ERCOT. Based on the estimated load profiling data, we observe a significant rising proportion of residential load sectors with the winter storm incoming (Fig.~\ref{fig:data_and_model}-a), which should have varied in the range between 10\% to 50\% under normal conditions. Note that the distinct pattern in Far West is mainly due to its sparse population. It is worth remarking that load profiling is critical for demand response assessment, since different demand response programs may have distinct performance that is determined real-time electricity demand of load sectors under specific scenarios.

\subsection*{Simulation Model Creation and Calibration}
This paper uses the synthetic 2,000-bus Texas grid model used for our previous preliminary study~\cite{wu2021open}, which is adapted from~\cite{breakthrough_data} and rigorously calibrated in several aspects, namely, system topology, transmission lines rating, generation units capacity, and geographical demand distribution. The topology of the synthetic 2,000-bus Texas grid was originally presented in~\cite{birchfield2017grid}. Transmission line capacity ratings and impedance have been updated to properly incorporate the 2021 generation mix and demand distribution. Generator capacities have been updated to incorporate the installed generation capacity data~\cite{eia_capacity} from 2016 to 2021. The loads of weather zones have been updated in order to reflect the up-to-date data~\cite{ercot_gridinfo}. We additionally decompose the loads into multiple sectors by utilizing the load profiling data, which can be used for load shedding allocation.
To give an intuitive impression, we visualize the topology of the synthetic grid in Fig.~\ref{fig:data_and_model}-b, where the width of branches is proportional to the corresponding transmission line capacity.
% The topology of the synthetic 2,000-bus Texas grid was originally presented in~\cite{birchfield2017grid}. While maintaining the original topology, transmission line capacity ratings and impedances have been updated, in~\cite{breakthrough_data} and~\cite{wu2021open} successively, to properly incorporate the 2021 generation mix and demand distribution. Running direct current optimal power flow (DCOPF) simulations, transmission line parameters are adjusted to ensure network feasibility and avoid non-realistic curtailment of renewable generation due to congestion.

% Generator capacities originally specified in~\cite{birchfield2017grid} have been updated in~\cite{breakthrough_data} and~\cite{wu2021open} to incorporate data from between 2016 and 2021. In~\cite{breakthrough_data}, the largest generators integrated to the system between 2017 and 2019 are added to the synthetic grid model and the generation mix is scaled to appropriately reflect data from the start of 2020. In~\cite{wu2021open}, the generators in the synthetic grid are updated to correspond to data from the beginning of 2021; this includes adding of eight new generators, all connected to high-voltage buses near their actual locations, and scaling the existing generator fleet so that totals by generation type and weather zone match those in EIA Form 860-M, December 2020.

% Electric demand is distributed from the publicly available aggregate weather zone demand to load buses in the synthetic grid using the method outlined in~\cite{birchfield2017grid}. The aggregate weather zone demand is updated in both~\cite{breakthrough_data} and~\cite{wu2021open} in order to reflect the up-to-date data.

% \textcolor{red}{XT: @Lane, @Bainan, could you please add brief introduction of the synthetic grid? (most of details are the same as last year's). LS: I believe this should be done now. Please let me know if you had something else in mind.}







==> sec/4_Baseline.tex <==



\begin{figure}[htpb!]
	\centering
	\includegraphics[width=0.5\columnwidth]{fig/curve_reproduction.pdf}
	\caption{Simulated load shedding curve with anatomy of components in comparison with the actual total shedding. Here L.S. means load shedding. Simulated total load shedding equals to the sum of simulated interruptible load and forced load shedding.}
	\label{fig:baseline_loadshedding}
\end{figure}

\section*{Baseline model of the 2021 Texas Blackout Event}\label{sec:baseline}
This section aims to (i) validate the proposed simulation model and methodology by reproducing the 2021 Texas blackout event and (ii) provide a baseline for the assessment of demand response portfolios.




\subsection*{Reproduction of the 2021 Texas Blackout Event}
To provide a baseline for demand response portfolios of interests, we reproduce the 2021 Texas blackout event from February 15 to February 18 with limited demand flexibility following the proposed model-based simulation. Here, we use the power system reliability index \textit{Energy-Not-Served} (ENS) as the metric to quantify the severity of the blackout event~\cite{singh2018electric}.
% Fig.~\ref{fig:baseline_loadshedding} shows the comparison between .

We demonstrate the fidelity of the simulation model and the designed load shedding algorithm by the good match between the actual and simulated total load shedding (Fig.~\ref{fig:baseline_loadshedding}) that represent a total of 998.8 GWh and 955.5 GWh ENS (4.33\% difference), respectively. The correlation coefficient between the two time series is 0.88, which also indicates a good match between the simulated load shedding process and actual ERCOT record. The unavoidable mismatch attributes to the combined effects of errors in synthetic grid modelling and system operation under emergency conditions.
The result also shows that the limited demand flexibility in the real-world grid has trivial effects on electricity scarcity mitigation under such extreme weather condition, stressing the necessity of facilitating demand response portfolios.


% In the remaining of the paper, the simulated load shedding in the baseline case will serve as a benchmark for demand response assessment.

% The limited demand flexibility in the 2021 Texas blackout event is trivial compared with the power shortage that once exceeded 20 GW, and it has run out when the system entered the EEA 3 stage.





==> sec/supplementary_figures.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Supplementary_Figures%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section*{Supplementary Figures}

\subsection*{Supplementary Figure 1: Synthetic Texas Electric Grid Model}
\begin{figure*}[thpb!]
	\centering
	\includegraphics[width=0.5\textwidth]{fig/simulation_model.pdf}
	\caption{Visualization of synthetic simulation models over weather zones. It shows the topology of the synthetic Texas grid adapted from~\cite{wu2021open}, where the width is proportional to the transmission line capacity.}
	\label{fig:data_and_model}
\end{figure*}


\clearpage

\subsection*{Supplementary Figure 2: Forced load shedding density distribution}
\begin{figure*}[htpb!]
	\centering
	\includegraphics[width=1\textwidth]{fig/DR_3in1_density.pdf}
	\caption{Density distributions of forced load shedding curves with demand flexibility of various mechanisms and scales, being supplementary information to the ENS metric. a,b, The peak of distribution becomes sharper and closer to zero along when the scales. c, Incentive-based demand response shows relatively lower sensitivity to the scale. Such observation also echos with the conclusion in the main text that merely developing incentive-based demand response cannot fully avoid electricity crisis due to the stochasticity and the limitation of inherent voluntary mechanism.}
	\label{fig:single-measure-density}
\end{figure*}
% To present what-if blackout events clearly and comprehensively in an alternative way, we perform kernel density estimation (KDE) to calculate the density distribution of load shedding amount, which can serve as a complement to the ENS metric. ab, We observe that for interruptible load and load rationing, the peak of distribution becomes sharper and closer to zero along with the scale. c, Incentive-based demand response shows relatively lower sensitivity to the scale (Fig.~\ref{fig:single-measure-density}-c). Such observation also echos with the conclusion in the main text that merely developing incentive-based demand response cannot fully avoid electricity crisis due to the stochasticity and the limitation of inherent voluntary mechanism.


\clearpage

\subsection*{Supplementary Figure 3: Contour of Up-Scaling Multiples of Interruptible Load with Varying Scales of Incentive-Based Demand Response and Residential Load Rationing}
\begin{figure*}[htpb!]
	\centering
	\includegraphics[width=0.5\textwidth]{fig/border_contour_2D.pdf}
	\caption{Contour of up-scaling multiples of interruptible load with varying scales of incentive-based demand response and residential load rationing, which can exactly avoid electricity outage.}
	\label{fig:contour}
\end{figure*}

% To present what-if blackout events clearly and comprehensively in an alternative way, we perform kernel density estimation (KDE) to calculate the density distribution of load shedding amount, which can serve as a complement to the ENS metric. We observe that for interruptible load and load rationing, the peak of distribution becomes sharper and closer to zero along with the scale (Fig.~\ref{fig:single-measure-density}-a and~\ref{fig:single-measure-density}-b), while that of incentive-based demand response shows relatively lower sensitivity to the scale (Fig.~\ref{fig:single-measure-density}-c). Such observation also echos with the conclusion in the main text that merely developing incentive-based demand response cannot fully avoid electricity crisis due to the stochasticity and the limitation of inherent voluntary mechanism. 

\clearpage


\subsection*{Supplementary Figure 4: Demand Flexibility Curves of Different Portfolios}
\begin{figure*}[htpb!]
	\centering
	\includegraphics[width=1\textwidth]{fig/curves_demand_response_ration.pdf}
	\caption{Demand flexibility provided by multiple mechanisms in different portfolios to exactly avoid electricity outage as supplementary information to Fig. 5 in the main text. a-c, Demand flexibility provided by incentive-based demand response (30$\%$, 40$\%$ and 50$\%$ coverage rate) and interruptible loads (790$\%$, 880$\%$ and 970$\%$ up-scaling rate), with no residential load rationing. d-f, Demand flexibility provided by incentive-based demand response (10$\%$, 20$\%$ and 30$\%$ coverage rate), interruptible loads (370$\%$, 590$\%$ and 530$\%$ up-scaling rate), and residential load rationing of 50$\%$ participation rate.}
	\label{fig:DR_portfolios_nonstacked_curves}
\end{figure*}

\clearpage

%\section*{Supplementary Tables}
%\clearpage

==> sec/supplementary_notes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Supplementary_Notes%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Supplementary Notes}


\subsection*{Supplementary Note 1: Brief Introduction of Demand Response Programs in Texas}
Demand flexibility is concretized by demand response programs of various forms that can change the energy consumption of end-use customers from normal patterns in response to certain commands or signals.~\cite{balijepalli2011review}
In most electricity markets in the United States, demand response providers (DRPs) are allowed to collect demand response commitments from customers and are treated as ``virtual generators” that can participate in real-time markets and/or provide operating reserves in the ancillary services markets.~\cite{Loadresource, Nyiso, Caiso}

Specifically, load resources in ERCOT can participate in the ancillary service market, which includes regulation up/down, non-spinning reserve service, and responsive reserve service (RRS). The bulk part of these services is attributed to the RRS, which can be automatically interrupted by under-frequency relays (UFRs) or manually cut-off within a ten-minute notice.~\cite{habib2021improving} During the most difficult hours of the Texas power outage, the maximum load reduction from load resources providing reserve was over 1,400 MW throughout the blackout event.~\cite{king2021timeline} 
Emergency Response Service (ERS) is another demand response program in the ERCOT, which will be activated during emergencies in the electric grid to avoid possible load shedding. There are two types of ERS with response times of 10 and 30 minutes procured by ERCOT four times a year.~\cite{drercot} 
Most demand response programs in ERCOT are focused on peak load reduction during summer. An essential example is the 4-Coincident Peak (4CP), where during each of the four months of June, July, August, and September, the single monthly system peak is set, and the 4CP charge for distribution
service providers are determined by calculating their load during ERCOT's monthly demand peak. 
Besides the demand response programs administered by ERCOT, there are also load management programs administered by Transmission and Distribution Service Providers (TDSP), which are an important source of demand flexibility. The three demand flexibility mechanisms considered in this paper cover most of these demand response programs. The ancillary services and the ERS are contractual interruptible loads, and 4CP is incentive-based demand response. One should note that although 4CP is a price-responsive demand response, in terms of structure and uncertainty, it is very similar to the coupon incentive-based demand response implemented in this paper. We obtain the available capacity of each demand response program in ERCOT from a presentation report,~\cite{drercot}  as follows. 
\begin{table}[tpbh!]
\centering
\begin{tabular}{|c|c|}
\hline
Demand response program & Capacity in ERCOT\\ \hline
Ancillary service market    & 2020 MW              \\ \hline
Emergency response service   & 1000 MW               \\ \hline
4-Coincident peak  & 2466 MW          \\ \hline
TDSP load management      & 300 MW          \\ \hline

\end{tabular}
% \caption{Assembled load profile data for estimating sector share}\label{tab:sector}
\end{table}


\clearpage

\subsection*{Supplementary Note 2: Details of Load Sector Share Estimation}
To improve the fidelity of our simulation and model different demand response proposals in richer detail, we further decompose the ERCOT weather-zone level total load data into 3 sectors: residential, commercial/industrial and municipal. We estimate a percentage share of the sectors in the total load of each weather zone, at each hour in February 2021 using the ERCOT backcasted actual load profile,~\cite{ERCOT_load_profiling} which contains normalized daily load profiles from each of the eight weather zones in ERCOT. The profile curves are produced using ERCOT load models which characterize the consumption pattern of loads in different sectors and with different sensitivity to weather and date-time variables. We first aggregate the consumption from all load model that belong to each sector and calculate the total daily variations for the February 2021 load profile data in each ERCOT weather zone. The sum of backcasted consumption of all models under each sector is the normalized to produce a timeseries of percentages. The hourly percentage timeseries are aligned with the historical hourly total consumption for each weather zone as shown in the table below, where $R_i$, $B_i$ and $O_i$ represent the percentage of consumption at hour $i$ for residential, business and other sector respectively. Note that, since each sector timeseries is normalized and scaled even in the raw ERCOT data, the percentages are of a hypothetical historic maximum MW capacity in each sector $[R_{max}, B_{max}, O_{max}]$ that is yet unknown (i.e. the MW consumption from the residential sector at hour $i$ should be $R_{max} * R_i$. For each hour, the estimated MW consumption from all 3 sectors, which is obtained by multiplying the total sector MW with the percentages ($R_i$, etc.), should sum up to the total historical MW consumption:
\begin{align}
R_i R_{max} + B_i B_{max} + O_i O{max} = P_i, \: \forall i
\end{align}
This formulation would allow us to use the data formatted in the table below to estimate the sector consumption through Non-Negative Least Square (NNLS), which gives the best estimation for the maximum sector MW consumption, $[R_{max}, B_{max}, O_{max}]$, from each sector and hence the hourly MW consumption from each sector.

\begin{table}[tpbh!]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Hour & Res. & Bus. & Oth. & Total MW \\ \hline
$T_1$        & $R_1$           & $B_1$        & $O_1$     & $P_1$             \\ \hline
$T_2$        & $R_2$           & $B_2$        & $O_t$     & $P_2$            \\ \hline
...        & ...             & ...          & ...       & ...             \\ \hline
$T_n$        & $R_n$           & $B_n$        & $O_n$     & $P_n$             \\ \hline
\end{tabular}
% \caption{Assembled load profile data for estimating sector share}\label{tab:sector}
\end{table}

\clearpage





\clearpage

